Cross-chain Deals and Adversarial Commerce

Modern distributed data management systems face a new challenge: how can autonomous, mutually-distrusting parties cooperate safely and effectively? Addressing this challenge brings up questions familiar from classical distributed systems: how to combine multiple steps into a single atomic action, how to recover from failures, and how to synchronize concurrent access to data. Nevertheless, each of these issues requires rethinking when participants are autonomous and potentially adversarial. We propose the notion of a *cross-chain deal*, a new way to structure complex distributed computations that manage assets in an adversarial setting. Deals are inspired by classical atomic transactions, but are necessarily different, in important ways, to accommodate the decentralized and untrusting nature of the exchange. We describe novel safety and liveness properties, along with two alternative protocols for implementing cross-chain deals in a system of independent blockchain ledgers. One protocol, based on synchronous communication, is fully decentralized, while the other, based on semi-synchronous communication, requires a globally shared ledger.

==> comments.tex <==
I have read through the paper and found a number of small
problems.


section 1.1

last para first sentence ending should be

   protocol that does not.

instead of

  protocol does not rely on synchrony.

there's a missing "that" right now, but also good to shorten
the sentence.

section 1.4

in title should it be "vs." instead of "vs" ? (assuming there's room!)

also in third bullet sentence 3:  I think it should be

   Alice compares ..

instead of

Alice's contract compares



section 2.2 after statement of property 1 it would be good if
the next sentence weren't indented. (like the sentence following
property 3)

Section 4.

post condition of transfer should include owns_C(P, a-a')

also I don't see any need for that footnote although certainly
not harmful.

section 4.1:

I think the second paragraph of commit phase ought to be
moved to validation phase.

and whether this moves or not, it would be nice to have
a blank after the first para. of commit phase (assuming there's room).

section 5.2

I think the expression "free loaders" is more common than
"free riders".  (riders appears several times.)

section 6.5 para 3. sentence 4 change

  Parties must engage ...

to

  Parties must list ...

or maybe Parties must identify or must provide

section 7

para 1. the second sentence should be

  The code shown here is not intended to be a detailed
  implementation; it is only ...

and the next sentence should start:

  To compare implementation costs, ...

remove para 2 (see below)

PROBLEM:

I think there is a problem with variable t in this section.
in 7.1 it is used to mean the total number of transfers
while in 7.2 it is used to mean the maximum number of transfers
occurring at one of the assets.

I think we need to do something about this but it isn't clear what.
I have suggested something below

section 7.1

Remove the first sentence of para 2.  Instead have a new para
(between current 1 and 2):

Figure 4 summarizes gas costs for a deal with n parties, m assets,
and t >= n transfers.

NOTE: I don't believe we have any assumption about how many transfers there
are as far as gas costs are concerned. just that there is a total
of t of them. (there is an assumption in the time costs see below).

Question: shouldn't the current figure 4 really be figure 3?

Section 7.1 Timelock protocol commit phase last sentence:
I think each party's vote is signed by up to n-1 others.

question: what is the meaning of "now" in figure 5?

in the CBC protocol commit phase:

this footnote should not appear in this section because
none of the code we are showing is for the CBC.

so either remove footnote 3 or maybe better it should
appear at the end of the first para of section 7.

section 7.2

the problem here is that "t" is used differently than it was in 7.1.
here it means the max. number of transfers done at any escrow.
Here's a potential fix.  the last sentence of first para of 7.2
becomes:

The results are summarized in Figure 7; here we assume each asset is
transferred k times.

AND change g to k in the figure.

(note: we can't say assets are transferred once because as defined
escrow doesn't include a transfer.)

I think the paper should still fit, and if necessary get rid of
footnote 1 or 3 or both.


section 8 para 1 sentence 2 "proved" should be "proven"

1.4
Changed to "the contract releases ..." since the contract does the comparing, not Alice herself


``now'' is the Solidity keyword that evaluates to the estimated current time. Changed font to look like a keyword.

The treatment of partial asset transfers was getting too complicated and distracting,
and no one else talks about transfers this way,
so I changed the text to say "asset (or set of assets) $a$".
That is, if a coin is divisible into 1000 atomic parts, then
transferring 5 milli-coins is transferring a set of 5 assets.

The Chicago manual of style says both "proved" and "proven" are acceptable, but "proved" is favored for past participles,
except that "proven" is favored for adjective proceeding the noun e.g., "proven remedy".

Figure 6 is CBC code. One of the referees was adamant we explain why we use Solidity code for non-PoW chains.

``Free rider'' is a technical term from economics, while ``freeloader'' is informal English implying moral judgment.

